Boosted Top Quarks and Jet Structure

The Large Hadron Collider (LHC) is the first machine that provides high enough energy to produce large numbers of boosted top quarks. The decay products of these top quarks are confined to a cone in the top quark flight direction and can be clustered to a single jet. Top quark reconstruction then amounts to analysing the structure of the jet and looking for subjets that are kinematically compatible with top quark decay. Many techniques have been developed recently to best use these topologies to identify top quarks in a large background of non-top jets. This article reviews the results obtained using LHC data recorded in the years 2010-2012 by the experiments ATLAS and CMS. Studies of Standard Model top quark production and searches for new massive particles that decay to top quarks are presented.

==> tools/boostedsymbols.tex <==
%
% User-defined latex commands for SUBSTRUCTURE
%

\RequirePackage{xspace}


% Jet mass related
\newcommand{\mjet}      {\ensuremath{m^{\rm jet}}\xspace}
\newcommand{\mlead}     {\ensuremath{\mjet_{1}}\xspace}
\newcommand{\mleadavg}  {\ensuremath{\langle\mlead\rangle}\xspace}
\newcommand{\Mjet}      {\ensuremath{m^{\rm jet}}\xspace}
\newcommand{\massjet}   {\mjet}
\newcommand{\mjetAvg}   {\ensuremath{\langle\mjet\rangle}\xspace}
\newcommand{\masstrkjet}{\ensuremath{m^{\rm track \; jet}}\xspace}

% Particle (and mass) related
\newcommand{\Wmass}     {\ensuremath{m_{\Wboson}}\xspace}
\newcommand{\WmassT}    {\ensuremath{m^{\Wboson}_{\rm T}}\xspace}
\newcommand{\topmass}   {\ensuremath{m_{t}}\xspace}
\newcommand{\mTransv}   {\ensuremath{m_{\rm T}}\xspace}
\newcommand{\massZprime}{\ensuremath{m_{\Zprime}}\xspace}

% Jet algorithm and grooming related
\newcommand{\akt}       {\antikt\xspace}
\newcommand{\Akt}       {\Antikt\xspace}
\newcommand{\aktfour}   {\antikt, \ensuremath{R=0.4}\xspace}
\newcommand{\AKTFat}    {\antikt, \ensuremath{R=1.0}\xspace}
\newcommand{\AKTPrune}  {\antikt, \ensuremath{R=1.0} (pruned)\xspace}
\newcommand{\AKTFilt}   {\antikt, \ensuremath{R=1.0} (filtered)\xspace}
\newcommand{\KTSix}     {\ensuremath{k_{T}}, \ensuremath{R=0.6}\xspace}
\newcommand{\kt}        {\ensuremath{k_{\rm T}}\xspace}
\newcommand{\kT}{\kt}
\newcommand{\Ca}        {Cambridge/Aachen\xspace}
\newcommand{\ca}     {\ensuremath{\mathrm{C/A}}\xspace}
\newcommand{\CASix}     {\CamKt, \ensuremath{R=0.6}\xspace}
\newcommand{\CAFat}     {\CamKt, \ensuremath{R=1.2}\xspace}
\newcommand{\CAPrune}   {\CamKt, \ensuremath{R=1.2} (pruned)\xspace}
\newcommand{\CAFilt}    {\CamKt, \ensuremath{R=1.2} (filtered)\xspace}
\newcommand{\SISCone}   {SISCone}
\newcommand{\SISConeSiz}{\SISCone, \ensuremath{R=0.6}\xspace}
\newcommand{\minKt}     {\ensuremath{\min\left(\pti^2, \ptj^2\right)}\xspace}
\newcommand{\minAKt}    {\ensuremath{\min\left(\pti^{-2}, \ptj^{-2}\right)}\xspace}
\newcommand{\minGen}    {\ensuremath{\min\left(\pti^{2p}, \ptj^{2p}\right)}\xspace}
\renewcommand{\pt}      {\ensuremath{p_{\rm T}}\xspace}
\renewcommand{\pttrue}  {\ensuremath{p_{\rm T}^{\rm true}}\xspace}
\newcommand{\Rij}       {\ensuremath{R_{ij}}\xspace}
\newcommand{\DR}      {\ensuremath{\Delta R}\xspace}
\newcommand{\DRij}      {\ensuremath{\Delta\Rij}\xspace}
\newcommand{\DRratio}   {\ensuremath{\frac{(\DRij)^2}{R^2}}\xspace}
\newcommand{\diB}       {\ensuremath{d_{iB}}\xspace}
\newcommand{\Rfilt}     {\ensuremath{R_{\rm filt}}\xspace}
\newcommand{\Nfilt}     {\ensuremath{N_{\rm filt}}\xspace}
\newcommand{\sjone}     {\ensuremath{j_{1}}\xspace}
\newcommand{\sjtwo}     {\ensuremath{j_{2}}\xspace}
\newcommand{\msubjone}  {\ensuremath{m^{\sjone}}\xspace}
\newcommand{\msubjtwo}  {\ensuremath{m^{\sjtwo}}\xspace}
\newcommand{\ptsubjone} {\ensuremath{\pt^{\sjone}}\xspace}
\newcommand{\ptsubjtwo} {\ensuremath{\pt^{\sjtwo}}\xspace}
\newcommand{\Rsubjets}  {\ensuremath{R_{\sjone,\sjtwo}}\xspace}
\newcommand{\DRsubjets} {\ensuremath{\Delta\Rsubjets}\xspace}
\newcommand{\Nsubjet}   {\ensuremath{N_{\rm subjet}}\xspace}
\newcommand{\pti}       {\ensuremath{p_{{\rm T}i}}\xspace}
\newcommand{\ptj}       {\ensuremath{p_{{\rm T}j}}\xspace}
\newcommand{\ycut}      {\ensuremath{y_{\rm cut}}\xspace}
\newcommand{\mcut}      {\ensuremath{m_{\rm cut}}\xspace}
\newcommand{\ymin}      {\ensuremath{y_{\min}}\xspace}
\newcommand{\fcut}      {\ensuremath{f_{\rm cut}}\xspace}
\newcommand{\Rsub}      {\ensuremath{R_{\rm sub}}\xspace}
\newcommand{\drsub}     {\ensuremath{\Rsub}\xspace}
\newcommand{\mufrac}    {\ensuremath{\mu_{\rm frac}}\xspace}
\newcommand{\rcut}      {\ensuremath{R_{\rm cut}}\xspace}
\newcommand{\zcut}      {\ensuremath{z_{\rm cut}}\xspace}
\newcommand{\largeR}    {large-\ensuremath{R}\xspace}
\newcommand{\LargeR}    {Large-\ensuremath{R}\xspace}


% Insitu mass validation
\newcommand{\rtrkjet}       {\ensuremath{r_{\rm track \; jet}}\xspace}
\newcommand{\rtrkjetPt}     {\ensuremath{\rtrkjet^{\pt}}\xspace}
\newcommand{\rtrkjetM}      {\ensuremath{\rtrkjet^{m}}\xspace}
\newcommand{\AvgrtrkjetM}   {\ensuremath{\langle\rtrkjet^{m}\rangle}\xspace}
\newcommand{\rtrkjetPtData} {\ensuremath{\rtrkjet^{\pt,{\rm data}}}\xspace}
\newcommand{\rtrkjetMData}  {\ensuremath{\rtrkjet^{m,{\rm data}}}\xspace}
\newcommand{\rtrkjetPtMC}   {\ensuremath{\rtrkjet^{\pt,{\rm MC}}}\xspace}
\newcommand{\rtrkjetMMC}    {\ensuremath{\rtrkjet^{m,{\rm MC}}}\xspace}
\newcommand{\RtrkjetPt}     {\ensuremath{R_{r{\rm \; track \; jet}}^{\pt}}\xspace}
\newcommand{\RtrkjetM}      {\ensuremath{R_{r{\rm \; track \; jet}}^{m}}\xspace}

% Jet substructure related
\newcommand{\shapeV}    {\ensuremath{{\cal V}}\xspace}
\newcommand{\htt}       {HEP\-Top\-Tagger\xspace}
\newcommand{\subjetpt}  {\ensuremath{\pT^{\rm subjet}}\xspace}
\newcommand{\subjetptl} {\ensuremath{\pT^{\rm subjet, lead}}\xspace}
\newcommand{\subjetptsl}{\ensuremath{\pT^{\rm subjet, sublead}}\xspace}
\newcommand{\yij}       {\ensuremath{y_{ij}}\xspace}
\newcommand{\dcut}      {\ensuremath{d_{\rm cut}}\xspace}
\newcommand{\dmin}      {\ensuremath{d_{\min}}\xspace}
\newcommand{\dij}       {\ensuremath{d_{ij}}\xspace}
\newcommand{\Dij}       {\ensuremath{\sqrt{\dij}}\xspace}
\newcommand{\DOneTwo}   {\ensuremath{\sqrt{d_{12}}}\xspace}
\newcommand{\DTwoThr}   {\ensuremath{\sqrt{d_{23}}}\xspace}
\newcommand{\xj}        {\ensuremath{x_{J}}\xspace}
\newcommand{\jetFunc}   {\ensuremath{J^{(eik),c} (\mjet, \pT, R)}\xspace}
\newcommand{\tauN}      {\ensuremath{\tau_N}\xspace}
\newcommand{\tauOne}    {\ensuremath{\tau_{1}}\xspace}
\newcommand{\tauTwo}    {\ensuremath{\tau_{2}}\xspace}
\newcommand{\tauThr}    {\ensuremath{\tau_{3}}\xspace}
\newcommand{\tauTwoOne} {\ensuremath{\tau_{21}}\xspace}
\newcommand{\tauThrTwo} {\ensuremath{\tau_{32}}\xspace}
\newcommand{\dip}       {\ensuremath{\mathcal{D}}\xspace}
\newcommand{\dipOneTwo} {\ensuremath{\dip_{12}}\xspace}
\newcommand{\dipTwoThr} {\ensuremath{\dip_{23}}\xspace}
\newcommand{\dipOneThr} {\ensuremath{\dip_{13}}\xspace}
\newcommand{\COneThr}   {\ensuremath{C_{1}^{(3)}}\xspace}

% Samples
\newcommand{\Zprimett}  {\ensuremath{Z'\ra t\bar{t}}\xspace}
\newcommand{\Zqq}       {\ensuremath{Z\ra q\bar{q}}\xspace}
\newcommand{\Wqq}       {\ensuremath{W\ra q\bar{q}}\xspace}


% Random
\newcommand{\mpi}       {multiple parton interactions\xspace}

\newcommand{\DRmin}     {\ensuremath{\Delta{R}_{\rm min}}\xspace}

\newcommand{\avg}[1]{\left< #1 \right>} % for e.g. <\mu>

\newcommand{\Delphes}{Delphes\xspace}
\newcommand{\delphes}{\Delphes}
\newcommand{\herwig}{HERWIG\xspace}
\renewcommand{\geant}{GEANT4\xspace}
%\newcommand{\herwigpp}{HERWIG++\xspace}
\newcommand{\madgraph}{MadGraph\xspace}
\newcommand{\sherpa}{SHERPA\xspace}
\newcommand{\PGS}{PGS\xspace}
\newcommand{\acerdet}{AcerDET\xspace}
\newcommand{\acermc}{AcerMC\xspace}
\newcommand{\pythia}{\Pythia}
\newcommand{\powheg}{POWHEG\xspace}
\newcommand{\powhegpythia}{POWHEG+PYTHIA\xspace}
\newcommand{\alpgen}{ALPGEN\xspace}
\newcommand{\alpgenherwig}{ALPGEN+HERWIG\xspace}
\newcommand{\alpgenpythia}{ALPGEN+PYTHIA\xspace}
\newcommand{\mcatnlo}{MC@NLO\xspace}
\newcommand{\hathor}{HATHOR\xspace}
\newcommand{\amegicpp}{AMEGIC++\xspace}
\newcommand{\madgraphpythia}{MadGraph+PYTHIA\xspace}
\newcommand{\madgraphherwigpp}{MadGraph+HERWIG++\xspace}


\renewcommand{\pt}     {\ensuremath{p_{\rm T}}\xspace}
\renewcommand{\et}     {\ensuremath{E_{\rm T}}\xspace}
\renewcommand{\pT}{\pt}
\renewcommand{\ET}{\et}
\newcommand{\etaphi}     {\ensuremath{(\eta, \phi)}\xspace}
\renewcommand{\bbbar}{\ensuremath{b\bar{b}}\xspace}
\newcommand{\mtt}{\ensuremath{m_{t\bar{t}}}\xspace}
\renewcommand{\ttbar}{\ensuremath{t\bar{t}}\xspace}
\renewcommand{\bjets}{$b$-jets\xspace}
\newcommand{\jht}{Johns Hopkins Top Tagger\xspace}
\newcommand{\ETmiss}{\mbox{\ensuremath{\slash{\!\!\!\!E_{\rm T}}}}\xspace}
\renewcommand{\Zprime}{\ensuremath{Z'}\xspace}
\newcommand{\gKK}{\ensuremath{g_{\rm KK}}\xspace}
\newcommand{\ttt}{Top Template Tagger\xspace}
\newcommand{\lpjets}{lepton+jets\xspace}
\newcommand{\Wpjets}{$W\!$+jets\xspace}
\newcommand{\Zpjets}{$Z\!$+jets\xspace}
\newcommand{\Wpb}{$W\!\!+\!b$\xspace}
\newcommand{\DeltaReta}{\ensuremath{\DeltaR_{\eta}}\xspace}
\newcommand{\DeltaRij}{\ensuremath{\DeltaR_{ij}}\xspace}
\newcommand{\DeltaROneTwo}{\ensuremath{\DeltaR_{12}}\xspace}

\newcommand{\httA}{U}
\newcommand{\httB}{V}
\newcommand{\httC}{W}
\newcommand{\httD}{X}
\newcommand{\httE}{Y}
\newcommand{\httF}{Z}
\newcommand{\ovthree}{\ensuremath{OV_3}\xspace}
\newcommand{\Dcut}{\ensuremath{D_{\rm cut}}\xspace}
\newcommand{\sqrts}{\ensuremath{\sqrt{s}}\xspace}
\newcommand{\mw}{\ensuremath{m_W}\xspace}
\newcommand{\mt}{\ensuremath{m_t}\xspace}
\newcommand{\ptt}{\ensuremath{p_{{\rm T},t}}\xspace}
%\newcommand{\avmu}{\ensuremath{\langle \mu \rangle}\xspace}
\newcommand{\avmu}{\ensuremath{\mu}\xspace}
\newcommand{\instL}{\ensuremath{\mathcal{L}}\xspace}
%\newcommand{\Npv}{\ensuremath{N{\rm PV}}\xspace}
%\newcommand{\rtrk}             {\ensuremath{r_{\rm trk}}\xspace}
\newcommand{\rtrkjetpt}{\ensuremath{r^{p_{\rm T}}_{\rm track\,jet}}\xspace}
\newcommand{\rtrkjetm}{\ensuremath{r^m_{\rm track\,jet}}\xspace}
%\newcommand{\Rtrk}             {\ensuremath{R_{\rm trk}}\xspace}
\newcommand{\Rtrkjetpt}{\ensuremath{R_{\rm track\,jet}^{\pt}}\xspace}
\newcommand{\Rtrkjetm}{\ensuremath{R_{\rm track\,jet}^{m}}\xspace}
\newcommand{\Rtrkaw}             {\ensuremath{\bar{R}^{\rm w}_{\rm trk}}\xspace}
\newcommand{\ptsubjet}{\ensuremath{p_{\rm T}^{\rm subjet}}\xspace}
\newcommand{\ptrel}{\ensuremath{p_{\rm T}^{\rm rel}}\xspace}
\newcommand{\njet}{\ensuremath{N_{\rm jet}}\xspace}
\newcommand{\nsub}{\ensuremath{N_{\rm sub}}\xspace}
\newcommand{\lsp}{\ensuremath{\tilde{\chi}^0_1}\xspace}
\newcommand{\sumfjm}{\ensuremath{M_J^\Sigma}\xspace}
\newcommand{\sqrtHT}{\ensuremath{\sqrt{H_{\rm T}}}\xspace}
\renewcommand{\HT}{\ensuremath{H_{\rm T}}\xspace}
\newcommand{\sqrtGeV}{\ensuremath{\sqrt{\!\!\GeV}}\xspace}
\newcommand{\ETmSignif}{\ensuremath{\ETmiss/\sqrtHT}\xspace}
\newcommand{\pTi}{\ensuremath{p_{{\rm T},i}}\xspace}
\newcommand{\pTj}{\ensuremath{p_{{\rm T},j}}\xspace}
\newcommand{\hptt}{HPT\-Top\-Tagger\xspace}
\newcommand{\http}{HEP\-Top\-Tagger$'$\xspace}
\newcommand{\fastjet}{FastJet\xspace}
\newcommand{\qjets}{Q-jets\xspace}
\newcommand{\ttH}{\ensuremath{t\bar{t}H}\xspace}
\newcommand{\Mpl}{\ensuremath{M_{\rm Pl}}\xspace}
\newcommand{\Lagr}{\ensuremath{\mathscr{L}}\xspace}
\newcommand{\dslash}{\mbox{\ensuremath{\slash{\!\!\!\partial}}}\xspace}
\newcommand{\fwidth}{\ensuremath{f_{\rm W}}\xspace}

